Adaptive Oracle-Efficient Online Learning

The classical algorithms for online learning and decision-making have the benefit of achieving the optimal performance guarantees, but suffer from computational complexity limitations when implemented at scale. More recent sophisticated techniques, which we refer to as oracle-efficient methods, address this problem by dispatching to an offline optimization oracle that can search through an exponentially-large (or even infinite) space of decisions and select that which performed the best on any dataset. But despite the benefits of computational feasibility, oracle-efficient algorithms exhibit one major limitation: while performing well in worst-case settings, they do not adapt well to friendly environments. In this paper we consider two such friendly scenarios, (a) "small-loss" problems and (b) IID data. We provide a new framework for designing follow-the-perturbed-leader algorithms that are oracle-efficient and adapt well to the small-loss environment, under a particular condition which we call approximability (which is spiritually related to sufficient conditions provided by Dud\'{i}k et al., [2020]). We identify a series of real-world settings, including online auctions and transductive online classification, for which approximability holds. We also extend the algorithm to an IID data setting and establish a "best-of-both-worlds" bound in the oracle-efficient setting.

==> alg.tex <==
\section{GFTPL with Small-Loss Bound}
\label{section:alg}
In this section, forgoing computational complexity,
we provide a new FTPL type of algorithm that enjoys the small-loss bound. We then show that the proposed algorithm can be  implemented  efficiently  by the offline oracle in Section \ref{imp-real}. Before diving into the details, we first briefly recall the definition of online learning and regret.

\paragraph{Preliminaries.} The online decision problem we consider can be described as follows. In each round $t$, a learner picks an action $x_t\in\X=[x^{(1)},\dots,x^{(K)}]$. After observing the adversary's decision $y_t\in\Y$, the learner suffers a loss $f(x_t,y_t)$ where the loss function $f:\X\times\Y\mapsto[0,1]$ is known. The regret is defined as 
$$ R_T := \textstyle \E\left[\sum_{t=1}^T f(x_t,y_t) - L_T^* \right],$$
where $L_T^*=\min\limits_{k\in[K]}\sum_{j=1}^{T}f(x^{(k)},y_j)$ is the cumulative loss of the best action in hindsight, and the expectation is taken with respect to the potentially randomized strategy of the learner.

Our proposed= algorithm follows the framework of GFTPL \citep{dudik2020oracle}. 
To help understanding, we first give a brief introduction to the intuition behind this method. Specifically, in each round $t$, GFTPL picks $x_t$ by solving the following optimization problem:
$$ \textstyle x_t = \argmin\limits_{k\in [K]}\sum_{j=1}^{t-1} f(x^{(k)},y_j) + \left<\Gamma^{(k)},\alpha\right>,$$
where $\alpha$ is a $N$-dimensional noise vector ($N\ll K$)  generated from a uniform distribution, and $\Gamma^{(k)}$ is the $k$-th row of a matrix $\Gamma\in[0,1]^{K\times N}$, which is referred to as the \emph{perturbation translation matrix} (PTM). Compared to vanilla FTPL, GFTPL only generates a small number ($N$) of random variables, and each expert is perturbed by a different linear combination of these random variables based on $\Gamma$. The results of \cite{dudik2020oracle} rely on the following assumption on $\Gamma$.   
\begin{defn}
    \textbf{{\emph{($\delta$-admissibility \citep{dudik2020oracle}}})} Let $\Gamma\in[0,1]^{K\times N}$ be a  matrix, and denote $\Gamma^{(k)}$ as the $k$-th row of $\Gamma$, and $\Gamma^{(k,i)}$ the $i$-th element of $\Gamma^{(k)}$.
    Then, $\Gamma$ is $\delta$-admissible if (a) $\forall k,k'\in[K]$, $\exists i\in[N]$, such that $\Gamma^{(k,i)}\not=\Gamma^{(k',i)}$; and (b) $\forall i\in[N], k,k'\in[K]$, such that $\Gamma^{(k,i)}\not=\Gamma^{(k',i)}$, then $|\Gamma^{(k,i)}-\Gamma^{(k',i)}|\geq \delta$.
\end{defn}
The $\delta$-admissibility guarantees that every two rows in $\Gamma$ are significantly distinct. As pointed out by \cite{dudik2020oracle}, this is the essential property required by GFTPL, and is used to \emph{stabilize} the algorithm in the analysis, i.e., ensuring that $\P[x_t\not=x_{t+1}]$ is small. However, motivated by adaptive FTPL in the inefficient setting \citep{hutter2005adaptive}, we observe that the small-loss bound can not rest on this notion of stability, instead one needs to control the following $\forall t$ and $\forall i\in[K]$,
\begin{equation}
\label{eqn:key-ratio}
    \frac{\P[x_t=x^{(i)}]}{\P[x_{t+1}=x^{(i)}]},
\end{equation}
the ratio of the probability of picking the $i$-th decision in two consecutive rounds. We note that $\delta$-admissibility is not strong enough to ensure this quantity is bounded, as we establish in the following lemma. (See  Appendix \ref{app:proof:lemma:1} for proof). 
\begin{lemma}
\label{lem:admis}
There is an instance of a $\delta$-admissible $\Gamma$, and a sequence $\{y_t: t=1, 2, \ldots \}$, such that if we run GFTPL we can have $\frac{\P[x_t=x^{(i)}]}{\P[x_{t+1}=x^{(i)}]}=\infty$ for some $i \in [K]$ and some $t > 0$.
\end{lemma}
To tackle this problem, we propose a new property for $\Gamma$. Let $B_\gamma^1 := \{ s \in \R^N : \|s\|_1 \leq \gamma \}$.  
\begin{defn}
\label{ass:single-out}
    \textbf{{\emph{($\gamma$-approximability)}}} Let $\Gamma\in[0,1]^{K\times N}$. We say that $\Gamma$ is \emph{$\gamma$-approximable} if $$\forall k \in [K], y \in \Y  \; \exists s \in B_\gamma^1 \, \forall j\in [K]: \quad \quad  \left<\Gamma^{(k)} - \Gamma^{(j)}, s \right> \geq f(x^{(k)},y)-f(x^{(j)},y).$$ 
\end{defn}
It may not be immediately obvious how we arrived at this condition, so let us provide some intuition. The goal of perturbation methods in sequential decision problems, going back to the early work of \citet{hannan1957approximation}, is to ensure that the algorithm is ``hedging'' across all available alternative decisions. A new observed data point $y$ may make expert $j$ suddenly look more attractive than expert $k$, as we have now introduced a new gap $f(x^{(k)},y)-f(x^{(j)},y)$ in their measured loss values. With this in mind, we say that $\Gamma$ is a ``good'' (i.e. approximable) choice for the PTM, if this gap can be overcome (hedged) by some small (i.e. likely) perturbation $s$, so that $\left<\Gamma^{(k)} - \Gamma^{(j)}, s \right>$ makes up the difference.
% Intuitively, this property means that, $\Gamma s_t^{(k)}$ is a good approximation of the loss vector $f(\cdot,y_t)$, in the sense that 
% it can simulate the loss gap between the $k$-th expert and other experts. The \emph{inequality} makes this property  flexible: We only need the gap approximation from above.
Later, we will show that $\gamma$-approximability guarantees the required stability measure in \eqref{eqn:key-ratio}, and thus is critical for the small-loss bound. 
% Before that, we make a comparison between our proposed condition and $\delta$-admissibility. 

We want to emphasize two final points. First, the $\gamma$-approximability condition is \emph{purely for analysis purposes} and we need not compute the $s$ in response to $y$ and $k$. Second, much of the computational and decision-theoretic challenges rest heavily on the careful design of $\Gamma$. The PTM allows the algorithm to perform the appropriate hedging across an exponentially-sized set of experts with only an $N \ll K$ dimensions of perturbation. As we demonstrate in the following example, we can always construct a $\gamma$-approximable $\Gamma$, with $N = O(\log K)$, but at the expense of computational efficiency. The proposed $\Gamma$ will not generally be \emph{compatible} with the given oracle.

\paragraph{Simple Example} For any online learning problem we may construct $\Gamma$ as follows. Let $N := \lceil \log_2 K \rceil$, and define the $k$th row $\Gamma^{(k)}$ to be the \emph{binary representation} of the index $k$, with $+1/-1$ values instead of $0/1$. We claim that this $\Gamma$ is $\gamma$-approximable, for $\gamma = \lceil \log_2 K \rceil$. We can satisfy the condition of Definition~\ref{ass:single-out}, by setting $s = \Gamma^{(k)}$. It is easy to that for any $j \ne k$ we have $\left<\Gamma^{(k)} - \Gamma^{(j)}, s \right> = \left<\Gamma^{(k)} - \Gamma^{(j)}, \Gamma^{(k)} \right> \geq 2 \geq f(x^{(k)},y)-f(x^{(j)},y)$, where the last inequality holds because $|f(x^{(i)},y)| \leq 1$ for any $i \in [K]$.



\paragraph{Comparison} We note that, although $\gamma$-approximability leads to a much tighter bound, it is not stronger than $\delta$-admissibility. Instead, they are incomparable conditions. Specifically:
\begin{itemize}
\item In Section \ref{subsection:auction} we demonstrate that when $\Gamma$ is binary, 
admissibility leads to approximability. As shown by \cite{dudik2020oracle}, a binary and admissible $\Gamma$ exists in various online auctions problems, including VCG with bidder-specific reserves \citep{roughgarden2019minimizing}, envy-free item pricing 
\citep{guruswami2005profit}, online welfare maximization in multi-unit auction \citep{dobzinski2010mechanisms}, and simultaneous second-price auctions \citep{daskalakis2016learning}. We can directly obtain an approximable $\Gamma$ in such cases.
\item On the other hand, in problems such as level auction \citep{dudik2020oracle}, one can construct both admissible and approximable $\Gamma$, although in different ways; we discuss in Section \ref{subsection:auction}.
\item In section \ref{subsection:other:application}, we show that, when the adversary's action space is small, we can always construct a $\gamma$-approximable $\Gamma$, while $\delta$-admissible $\Gamma$ in general does not exist. 
  \item In  Appendix \ref{app:counter:app}, we show that in some cases a $\delta$-admissible $\Gamma$ can be obtained while $\gamma$-approximability cannot be achieved. 
\end{itemize}
\begin{algorithm}[t]
\caption{Generalized follow-the-perturbed-leader with small-loss bound}
\begin{algorithmic}[1]
\label{alg:GFTPL:main}
\STATE \textbf{Init:} $\Gamma\in[0,1]^{K\times N}$
% , seq. $\{\eta_t > 0 : t=1, 2, \ldots \}$
\STATE Draw IID vector $\alpha=[\alpha^{(1)},\dots,\alpha^{(N)}] \sim \text{Lap}(1)^N$; that is, $p(\alpha^{(i)})=\frac{1}{2}\exp(-|\alpha^{(i)}|)$
\FOR{$t=1,\dots,T$}
\STATE Set $\alpha_t \gets \frac{\alpha}{\eta_t}$, where $\eta_t > 0$ a parameter computed online
\STATE Choose $ \displaystyle x_t \gets \argmin\limits_{k\in [K]}\sum_{j=1}^{t-1} f(x^{(k)},y_j) + \left<\Gamma^{(k)},\alpha_t\right>$
\STATE Observe $y_t$
% where $\Gamma^{(k)}$ is the $k$-th row of $\Gamma$, $\alpha_t=\frac{\alpha}{\eta_t}$, and $\eta_t$ is a non-increasing step size. %\gw{By definition, $p(\alpha^{(k)}_t)=\frac{1}{2}\exp(-\eta_t|\alpha^{(k)}|)$.}
\ENDFOR
\end{algorithmic}
\end{algorithm}
Equipped with the $\gamma$-approximable PTM, we develop a generalized  follow-the-perturbed-leader algorithm with the Laplace distribution\footnote{Note that the Laplace distribution is not the unique choice to get the small-loss bound. In  Appendix \ref{app:proof:ellp}, we prove that the $\ell_p$ perturbation 
$
p(\alpha)\propto\exp\left\{-\left(\sum_i |\alpha^{(i)}|^p\right)^{\frac{1}{p}}\right\}
$
indeed works for any $p\geq 1$.} %However, as the $\ell_p$ perturbation does not lead to an improvement in the regret bound and the Laplace perturbation is easier to implement, we only discuss the Laplace perturbation in the main paper. } 
and a time-variant step size, which is summarized in Algorithm \ref{alg:GFTPL:main}. For the proposed algorithm, we successfully obtain the following  stronger stability property.  
% \begin{lemma}
\begin{restatable}{lemma}{primelemma}
\label{lem:main:1111}
Assume $\Gamma$ is $\gamma$-approximable. Let $x_t'=\argmin_{k\in[K]}\sum_{j=1}^t f(x^{(k)},y_j)+\left\langle \Gamma^{(k)},\alpha_t \right\rangle$.
Then in each round $t$, we have  $\forall i\in[K],$ 
$$\P[x_t=x^{(i)}]\leq \exp\left({\gamma\eta_t}\right) \P[x'_t=x^{(i)}].$$
\end{restatable}

%\begin{lemma}
%\label{lem:main:1111}
%Assume $\Gamma$ is $\gamma$-approximatable. Let $x_t'=\argmin_{k\in[K]}\sum_{j=1}^t f(x^{(k)},y_j)+\left\langle \Gamma^{(k)},\alpha \right\rangle$ be the infeasible leader at round $t$.
%Then in each round $t$, we have  
%$$\E[f(x_t,y_t)]\leq \exp\left(\frac{\gamma\eta_t}{\epsilon}\right) \E[f(x_t',y_t)].$$
%\end{lemma}
%To help understanding, in the following we provide a simple example for the case when $\Gamma$ is binary. In Section \ref{imp-real}, we will discuss how to construct a distinguishable $\Gamma$ in various real-world applications.
%\begin{example}
%Let $\Gamma\in[0,1]^{K\times N}$ be a binary matrix where every two rows are distinct by at least one element, then $\Gamma$ is $(N,1)$-distinguishable.
%\end{example}
Note that  we replace the term $x_{t+1}$ in \eqref{eqn:key-ratio} with $x_t'$, as a time-variant step-size is used.  Based on Lemma \ref{lem:main:1111}, we obtain the regret bound of Algorithm \ref{alg:GFTPL:main} as follows.
\begin{theorem}
\label{thm:main:11}
Assume $\Gamma$ is $\gamma$-approximable, and let $L_{T}^*=\min_{k\in[K]}\sum_{j=1}^{T}f(x^{(k)},y_j)$. Algorithm \ref{alg:GFTPL:main}, with $\eta_t=\min\left\{\frac{1}{\gamma},\frac{c}{\sqrt{L^*_{t-1}+1}}\right\}$ for any $c>0$, achieves the following regret bound: 
\begin{equation}
    \begin{split}
R_T\leq {} & \left(\frac{4\sqrt{2}\max\{2\ln K,\sqrt{N\ln K}\}}{c}
+{2\gamma}\left(c+\frac{1}{c}\right)\right) \sqrt{L_T^*+1}\\
{} & + {8\gamma}\ln\left(\frac{1}{c}\sqrt{L_T^*+1}+\gamma\right) + 2\gamma^2 + 4\sqrt{2}\max\{2\ln K,\sqrt{N\ln K}\}\gamma.
% \left(\frac{20}{c}\max\{\ln K,\sqrt{N\ln K}\}+{2\gamma}\left(c+\frac{1}{c}\right)\right) \sqrt{L_T^*+1}\\
% {} & + \frac{8\gamma}{c }\ln\left(\frac{1}{c}\sqrt{L_T^*+1}\right) + {10\gamma^2} + {20\gamma}\max\{\ln K,\sqrt{N\ln K}\}.
  \end{split}
\end{equation}

\end{theorem} 
The proof of Lemma \ref{lem:main:1111} and Theorem \ref{thm:main:11} can be found in Appendix \ref{app:proof:thm1}. By setting $c=\Theta(1)$, Theorem \ref{thm:main:11} implies that our proposed algorithm achieves  $O(\max\{{\gamma},\ln K, \sqrt{N\ln K}\}\sqrt{L_T^*})$ regret bound. 

\paragraph{Comparison to GFTPL \citep{dudik2020oracle}} The original GFTPL algorithm has an $O(\frac{N}{\delta}\sqrt{T})$ regret bound. For the dependence on $T$, our $O(\sqrt{L_T^*})$ bound reduces to $O(\sqrt{T})$ in the worst-case, and automatically becomes tighter when $L_T^*$ is small. On the other hand, for the dependence on other terms, we note that
both $\frac{N}{\delta}$ and $\max\{{\gamma},\ln K, \sqrt{N\ln K}\}$ are lower bounded by $\Omega(\ln K)$, and their exact relationship depends on the specific problem. In Section \ref{imp-real}, we show that for many auction applications, the two terms are on the same order. Moreover, in cases such as when $|\Y|$ is small,  Algorithm \ref{alg:GFTPL:main} with an appropriate $c$ leads to  $O\left(\sqrt{L_T^*\max\{\ln K,\sqrt{|\Y|\ln K}\}}\right)$ regret bound, while the regret bound of GFTPL in \cite{dudik2020oracle} can blow up since $\delta$ can be infinitely small.



%  We further note that the Laplace distribution is not the unique choice to get the small loss bound, as shown in the following Theorem.
 
%  In the Appendix \ref{app:proof:ellp}, we prove that the following $\ell_p$ perturbation 
% \begin{equation}
%     p(\alpha)\propto\exp\left\{-\left(\sum_i |\alpha^{(i)}|^p\right)^{\frac{1}{p}}\right\}
% \end{equation}
%  works for any $p\geq 1$. However, as the $\ell_p$ perturbation does not lead to an improvement in the regret bound and the Laplace perturbation is easier to implement, we only discuss the Laplace perturbation in the main paper. 

%\begin{cor}
%Assume $\Gamma$ is ($\gamma$,$\epsilon$)-distinguishable. For Algorithm 1 we have
%$$
%\lim_{L_T^{\star}\to\infty}\frac{\sum_{t=1}^T f(x_t,y_t)}{\sum_{t=1}^T f(x^{\star},y_t)}=\frac{\sum_{t=1}^T f(x_t,y_t)}{L_T^{\star}}=1.
%$$
% lim_{n\to\infty}
%\end{cor}

==> applications.tex <==
\section{Oracle-efficiency and Applications}
\label{imp-real}
In this section, we discuss how to run Algorithm \ref{alg:GFTPL:main} in an oracle-efficient way. Following \cite{dudik2020oracle}, we introduce the following  definition. 
\begin{defn}[Implementability]
\label{defn:imp}
A matrix $\Gamma$ is implementable with complexity $M$ if for each $j\in[N]$ there exists a dataset $S_j$, with $|S_j|\leq M$, such that $\forall k,k'\in[K]$, 
$$\Gamma^{(k,j)}-\Gamma^{(k',j)}=\sum_{(w,y)\in\S_j}w\left(f(x^{(k)},y)-f(x^{(k')},y)\right).$$
\end{defn}
Based on Definition \ref{defn:imp}, it is easy to get the following theorem, which is similar to Theorem 2.10 of \cite{dudik2020oracle}.
\begin{theorem}
If\ $\Gamma$ is implementable, then Algorithm \ref{alg:GFTPL:main} is oracle-efficient and has a a per-round complexity $O(T+NM)$.
\end{theorem}
In the following, we discuss how to construct approximable and implementable $\Gamma$ matrices in different applications. 
\subsection{Applications in online auctions}
\label{subsection:auction}
\begin{algorithm}[t]
\caption{Oracle-based GFTPL for the reward feedback}
\label{alg:GFTPL:33}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Data set $S_j$, $j\in[N]$, that implement a matrix  $\Gamma\in[0,1]^{K\times N}$, $\eta_1=\min\{\frac{1}{\gamma},1\}$.
\STATE Draw IID vector $\alpha=[\alpha^{(1)},\dots,\alpha^{(N)}] \sim \text{Lap}(1)^N$
\FOR{$t=1,\dots,T$}
\STATE Choose 
 $\displaystyle x_t \gets \argmin\limits_{k\in [K]}\sum_{j=1}^{t-1} f(x^{(k)},y_j) + \sum_{i=1}^N\frac{\alpha^{(i)}}{\eta_t}\left[\sum_{(w,y)\in \S_i}w\cdot r(x^{(k)},y)\right]$
\STATE Observe $y_t$
\STATE Compute ${\widehat{L}}_{t}^*=\min\limits_{k\in[K]}\sum_{j=1}^{t}f(x^{(k)},y_j)$ by using the oracle
\STATE Set $\eta_{t+1} \gets \min\left\{\frac{1}{\gamma},\frac{1}{\sqrt{\widehat{L}_t^*+1}}\right\}$ 
 %\gw{By definition, $p(\alpha^{(k)}_t)=\frac{1}{2}\exp(-\eta_t|\alpha^{(k)}|)$.}
\ENDFOR
\end{algorithmic}
\end{algorithm}
In this part, we apply Algorithm   \ref{alg:GFTPL:main} to  online auction problems, which is the main focus of \cite{dudik2020oracle}. To deal with this sort of problems, we first transform Algorithm \ref{alg:GFTPL:main} to  online learning with rewards setting, i.e., in each round $t$, after choosing $x_t$, instead of suffering a loss, the learner obtains a reward $r(x_t,y_t)\in[0,1]$. For this case, it is straightforward to see that running Algorithm \ref{alg:GFTPL:main} on a surrogate loss $f(x,y)=1-r(x,y)$ directly leads to the small-loss bound. To proceed, we slightly change this procedure and obtain Algorithm \ref{alg:GFTPL:33}. The main difference is that, we {{implement $\Gamma$ with the reward function $r(x,y)$, instead of the surrogate loss $f(x,y)$}}. This makes the construction of $\Gamma$ \emph{much easier}. We have the following regret bound for Algorithm \ref{alg:GFTPL:33}.
\begin{cor}
\label{cor:imp}
Let $f(x,y)=1-r(x,y)$. Assume $\Gamma$ is $\gamma$-approximable w.r.t. $f(x,y)$ and implementable with function $r(x,y)$. Then Algorithm \ref{alg:GFTPL:33}  is oracle-efficient and achieves the following regret bound: 
$$R_T= \E\left[L_T^*-\sum_{t=1}^Tr(x_t,y_t)\right]=O\left(\max\left\{\frac{\gamma}{\epsilon},\ln K, \sqrt{N\ln K}\right\}\sqrt{T-L_T^*}\right),$$
where $L_T^*=\max_{i\in[K]}\sum_{t=1}^T r(x^{(i)},y_t)$ is the cumulative reward of the best expert.
\end{cor}
 Next, we discuss how to construct the PTM in several auction problems.
%Finally, for auction problems, we introduce the following stronger data-independent version of Definition \ref{defn:imp}.
%\begin{defn}
%\label{ass:single-out}
%    \textbf{{\emph{($\gamma$-distinguishable)}}} Let $\Gamma\in[0,1]^{K\times N}$ be a  matrix, and denote $\Gamma^{(k)}$ as the $k$-th row of $\Gamma$. Then, $\Gamma$ is $\gamma$-distinguishable if\ $\forall k\in[K]$, $\exists s^{(k)}\in\R^{N}$, $\|s^{(k)}\|_{1}\leq \gamma$, such that $\left<\Gamma^{(k)}, s^{(k)}\right>\geq\left<\Gamma^{(j)}, s^{(k)}\right>+1$ for all rows $j\not=k$. 
%\end{defn}

%Note that since $f(x^{i},y_t)-f(x^{i},y_t)\leq1$ for all $i,j\in[K]$ and $t>0$, $\gamma$-distinguishablity directly leads to $\gamma$-approximability. 

\paragraph{Auctions with binary and admissible $\Gamma$.} As shown by \cite{dudik2020oracle}, in many online auction problems, such as VCG with bidder-specific reserves \citep{roughgarden2019minimizing}, envy-free item pricing 
\citep{guruswami2005profit}, online welfare maximization in multi-unit auction \citep{dobzinski2010mechanisms} and simultaneous second-price auctions \citep{daskalakis2016learning}, there exists a binary PTM which is  $1$-admissible and implementable with $N$ rows where $N\ll K$. For these cases, we have the following lemma. The proof is deferred to Appendix \ref{app:proof:binaryg}.
\begin{lemma}
\label{lem:binarygamma}
Let $\Gamma\in[0,1]^{K\times N}$ be a binary matrix and $1$-admissible, then $\Gamma$ is $N$-approximable.
\end{lemma}
Combining Lemma \ref{lem:binarygamma} with Corollary \ref{cor:imp}, and noticing the fact the $N=\Omega(\ln K)$, we can  obtain 
an $O(N\sqrt{T-L_T^*})$ bound for all of the above problems. Compared to the original GFTPL, our condition leads to a similar dependence on $N$ and a tighter dependence on $T$. More details about the aforementioned auction problems and corresponding regret bounds can be found in Appendix \ref{app:proof:auction}.

\subsection{Level auction}
\label{app:proof:level}
We consider the online level auction problem with single-item, $n$-bidders, $s$-level and $m$-discretization level. We give only a brief review of this problem setting, and we refer the reader to \citet{dudik2020oracle} for a complete description. In each round $t$ of this problem, firstly an auctioneer picks $s$ non-decreasing thresholds from a discretized set $\{\frac{1}{m},\dots,\frac{m}{m}\}$ for each bidder. Let $a_t=[a_t^{(1,1)},\dots,a_t^{(1,s)},\dots,a_t^{(n,1)},\dots,a_t^{(n,s)}]$ be the collection of the auctioneer's choices, where $a^{(i,j)}$ is $j$-th the threshold for the $i$-th bidder. Let $\A\in\{\frac{1}{m},\dots\frac{m}{m}\}^{ns}$ be all possible auctions. Following the distinct thresholds setting \citep{dudik2020oracle},  We further make the following assumption on $\A$. 
\begin{ass}
\label{ass:lebel:2}
Assume: (a) $\forall a,{a'}\in\mathcal{A}$, there  exists at least one pair $(i,j)\in [n]\times[s]$, such that $a^{(i,j)}\not={a'}^{(i,j)}$; and (b) $\forall a\in\mathcal{A}$, $\forall i\in[n]$, $a^{(i,1)}<\dots<a^{(i,s)}$.
\end{ass}
After $a_t$ is chosen, the bidders reveal their valuations. We denote the  collection of the bidders' valuations as $b_t=[b_t^{(1)},\dots,b_t^{(n)}]\in\B=[0,1]^n$. As a consequence, the auctioneer obtains a reward $r(a_t,b_t)$, which is calculated based on the following rule. 
\begin{defn}[The rule for level auction]
\label{defn:level}
For each bidder $i\in[n]$, define the level index $\ell_t^{(i)}$ be the maximum $j$ such that $a_t^{(i,j)}\leq b^{(i)}_t$, with $\ell_t^{(i)}=0$ when $a_t^{(i,1)}>b_t^{(i)}$. Then, all bidders with $0$ level index are eliminated (temporarily at round $t$). If no bidder left, $r(a_t,b_t)=0$. Otherwise, the bidder with the highest level index wins the item, and pays the price (i.e., $r(a_t,b_t)$) equal to the
minimum bid that he could have submitted and still won the auction. On the same level, the tie-break rule is in favor of the bidder with the smallest bidding index.
\end{defn}
In this framework the set of ``experts'' is the set $\A$ of threshold configurations over all bidders. The regret of the auctioneer over $T$ iterations is the gap between the revenue generated by the online choice of threshold configurations and the revenue of the best set of thresholds in hindsight, i.e.  
$$R_T := \E\left[\max_{a\in\A}\sum_{t=1}^T r(a,b_t)-\sum_{t=1}^Tr(a_t,b_t)\right].$$
%where $a^*=\argmax\limits_{k\in[K]}\sum_{t=1}^Tf(a^{(k)},b_t)$. Given any weighted adversarial decision set $\S=\{(w^{(j)},b^{(j)})\}_{j=1}^n$, the oracle 
%can solve the following offline optimization problem efficiently:
%$$\argmax\limits_{k\in[K]} \sum_{j=1}^n w^{(j)}f(a^{(k)},b^{(j)}).$$
\subsubsection{Algorithm and regret}

We first discuss how to construct an approximable (see Definition \ref{ass:single-out}) and implementable $\Gamma$ with small $\gamma$. Directly constructing $\Gamma$ is rather difficult. Thus, we first consider an \emph{augmented} auction problem with $n+1$ bidders. Let $\mathcal{A'}\in \{\frac{1}{m},\dots,\frac{m}{m}\}^{(n+1)s}$ be the set of possible auctions, and  $\mathcal{B'}\in[0,1]^{n+1}$ be the set of bidder profiles. We construct $\mathcal{A'}$ as follows:
%We firstly make the following assumptions on $\mathcal{P}$:
\begin{defn}
\label{ass:lebel}
(a) Distinct auctions (first $n$ bidders): $\forall a,{a'}\in\mathcal{A'}$, there  exists at least one pair $(i,j)\in [n]\times[s]$, such that $a^{(i,j)}\not={a'}^{(i,j)}$; (b) distinct thresholds (first $n$ bidders): $\forall a\in\mathcal{A'}$, $\forall i\in[n]$, $a^{(i,1)}<\dots<a^{(i,s)}$; and (c) fixed thresholds for the $(n+1)$-th bidder: $\forall a\in\mathcal{A'}$, $a^{(n+1,1)}=\frac{1}{m}$, $a^{(n+1,j)}=\frac{j-1}{m}$ for $j\in\{2,\dots,s\}$. 
\end{defn}
Comparing Assumption  \ref{ass:lebel:2} and Definition \ref{ass:lebel}, it can be seen that the elements in $\A'$ and $\A$ have an one-to-one correspondence: $\forall a\in\A$, there only exists one $a'\in\A'$, such that $\forall (i,j)\in[n]\times[s]$, $a^{(i,j)}=a'^{(i,j)}$, and vice versa. 

In the augmented problem, at each round $t$, firstly the auctioneer chooses $a'_t$ from $\A'$. At the same time, we let the bidders reveal $b_t'=[b_t;0]$, where $b_t$ is the bidder vector of the original problem, and $b_t'$ is a $(n+1)$-dimensional vector. Then, the  auctioneer obtain a reward $r'(a'_t,b_t')$, where $r': \A'\times \B'\mapsto [0,1]$ follows the auction rule in Definition \ref{defn:level}. For $a_t'$, denote the related auction in $\A$ as $a_t$, and we have the following lemma.
\begin{lemma}
We have $r(a_t,b_t)=r'(a'_t,b'_t)$, and 
$$\E\left[\max_{a\in\A}\sum_{t=1}^T r(a,b_t)-\sum_{t=1}^Tr(a_t,b_t)\right]=\E\left[\max_{a'\in\A'}\sum_{t=1}^T r'(a',b'_t)-\sum_{t=1}^Tr'(a'_t,b'_t)\right].$$
\end{lemma}
\begin{proof}
Since the last element of $b_t'$ is 0, so the $(n+1)$-th bidder will always be at the 0-th level when computing $r'(a'_t,b'_t)$, it will not change the reward at round $t$. We note that, it does not mean the augmentation is not useful: designing a PTM for $r'(a',b')$ is much easier than for the original problem.
% We could carefully design  $r'(a',b')$ when constructing the PTM to obtain approximability.
\end{proof}

This lemma reveals a duality between the two problems:
A low-regret and oracle-efficient algorithm for the augmented problem directly induces a low-regret and oracle-efficient  algorithm for the original problem by replacing $a'\in\A'$ with its corresponding auction $a_t$ in $\A$. To help understanding, we illustrate the relationship between the original problem and the augmented problem in Figure \ref{fig:la}.
\begin{figure}
\centering
  \includegraphics[width=0.8\linewidth]{lev-auc.pdf}
  \caption{The relationship between the original problem and the augmented problem.}
  \label{fig:la}
\end{figure}

Next, we propose 
to construct an approximable $\Gamma$ matrix for the augmented problem by using  $ns(m-s+1)$ elements of $\B'$. 
For $i\in\{1,\dots,n\}$, $j\in\{1,\dots,s\}$, and  $k\in\{1,\dots,m-s+1\}$, let a bidder vector $b'^{(i,j,k)}\in\B'$ be 
%be the bidder profile assigned for each column, and $\V$ the collection of $v$. Let $v[i,j,k]$ be
\begin{equation}
\label{eqn:v}
b'^{(i,j,k)}=\frac{k+j-1}{m}e_i+\frac{j-1}{m}e_{n+1},
\end{equation}
where $e_i$ is a $(n+1)$-dimension unit vector whose $i$-th element is 1 and all others are 0. 
We prove the following lemma. 
\begin{lemma}
\label{lem:level}
Let $\V=\{b'^{(i,j,k)}\}_{i,j,k}$ be the set containing all $b'$ defined in \eqref{eqn:v}. Let $\Gamma^{\V}\in[0,1]^{K\times ns(m-s+1)}$ be the matrix implemented from $\V$ by assigning each $r'(\cdot,b'^{(i,j,k)})$ to the columns of $\Gamma^{\V}$ one-by-one. Then $\Gamma^{\V}$ is $nsm$-approximable. 
\end{lemma}

\begin{table}[]
\centering
\caption{Illustration of $\Gamma^{\V}$ when $m=5$ and $s=3$. Each $a'^{(i,j)}$ is encoded by $m-s+1=3$ columns. Here $g=\frac{j-1}{m}=\frac{2-1}{5}=\frac{1}{5}$, and $h=\frac{j-1}{m}=\frac{3-1}{5}=\frac{2}{5}$. Consider the auctions whose $a'^{(i,2)}=\frac{3}{5}=\frac{k'+j-1}{m}=\frac{k'+1}{5}$. Then, at the second column  that is related to $a'^{(i,2)}$ (corresponds to $k'=2$), only such auctions can yield the highest revenue $\frac{3}{5}$, and the revenue is at least $\frac{1}{5}$ higher than auctions with $a'^{(i,2)}\neq\frac{3}{5}$.} 
\makeatletter
\label{tab:exp}
\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 1pt
    \futurelet \reserved@a \@xhline
}

\newcolumntype{"}{@{\hskip\tabcolsep\vrule width 1pt\hskip\tabcolsep}}
\makeatother
\resizebox{\columnwidth}{!}{\begin{tabular}{ccc"cccccccccccc}
\thickhline
  & \textbf{Auction $\mathbf{a'}$} &  &   & & & & \multicolumn{3}{c}{\textbf{Coding}} \\ \cline{5-13} 
\dots  & $(a'^{(i,1)},a'^{(i,2)},a'^{(i,3)})$ & \dots & \multicolumn{1}{l|}{\dots} &  & $a'^{(i,1)}$  &\multicolumn{1}{l|}{}  &  & $a'^{(i,2)}$  &\multicolumn{1}{l|}{} &  & $a'^{(i,3)}$  &\multicolumn{1}{l|}{} & \dots \\ 
\thickhline
\dots  & $(\unitfrac{1}{5},\unitfrac{2}{5},\unitfrac{3}{5})$ & \dots & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} & \unitfrac{1}{5} & \multicolumn{1}{l|}{\unitfrac{1}{5}} & \unitfrac{2}{5} & \unitfrac{2}{5} & \multicolumn{1}{l|}{\unitfrac{2}{5}}&  \unitfrac{3}{5}&  \unitfrac{3}{5} & \multicolumn{1}{l|}{ \unitfrac{3}{5}} & \dots\\ \hline 
\dots  & $(\unitfrac{1}{5},\unitfrac{2}{5},\unitfrac{4}{5})$ & \dots & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} & \unitfrac{1}{5}& \multicolumn{1}{l|}{\unitfrac{1}{5}} & \unitfrac{2}{5} & \unitfrac{2}{5} & \multicolumn{1}{l|}{\unitfrac{2}{5}}& h&  \unitfrac{4}{5}& \multicolumn{1}{l|}{ \unitfrac{4}{5}}& \dots\\\hline
\dots  &  $(\unitfrac{1}{5},\unitfrac{2}{5},\unitfrac{5}{5})$ & \dots  & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} & \unitfrac{1}{5}& \multicolumn{1}{l|}{\unitfrac{1}{5}} & \unitfrac{2}{5} & \unitfrac{2}{5} & \multicolumn{1}{l|}{\unitfrac{2}{5}}& h& h & \multicolumn{1}{l|}{ \unitfrac{5}{5}}& \dots\\\hline
\dots  &  $(\unitfrac{1}{5},\unitfrac{3}{5},\unitfrac{4}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} &\unitfrac{1}{5}& \multicolumn{1}{l|}{\unitfrac{1}{5}} & g & \unitfrac{3}{5} & \multicolumn{1}{l|}{\unitfrac{3}{5}}& h&  \unitfrac{4}{5}& \multicolumn{1}{l|}{ \unitfrac{4}{5}}& \dots\\\hline
\dots  &  $(\unitfrac{1}{5},\unitfrac{3}{5},\unitfrac{5}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} &\unitfrac{1}{5}& \multicolumn{1}{l|}{\unitfrac{1}{5}}& g& \unitfrac{3}{5} & \multicolumn{1}{l|}{\unitfrac{3}{5}}& h& h& \multicolumn{1}{l|}{ \unitfrac{5}{5}}& \dots\\\hline
\dots  &  $(\unitfrac{1}{5},\unitfrac{4}{5},\unitfrac{5}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & \unitfrac{1}{5} &\unitfrac{1}{5}& \multicolumn{1}{l|}{\unitfrac{1}{5}}& g& g& \multicolumn{1}{l|}{\unitfrac{4}{5}}& h& h& \multicolumn{1}{l|}{ \unitfrac{5}{5}}& \dots\\\hline
\dots &  $(\unitfrac{2}{5},\unitfrac{3}{5},\unitfrac{4}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & 0 &\unitfrac{2}{5}& \multicolumn{1}{l|}{\unitfrac{2}{5}}& g& \unitfrac{3}{5}& \multicolumn{1}{l|}{\unitfrac{3}{5}}& h&  \unitfrac{4}{5}& \multicolumn{1}{l|}{ \unitfrac{4}{5}}& \dots\\\hline
\dots &  $(\unitfrac{2}{5},\unitfrac{3}{5},\unitfrac{5}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & 0 &\unitfrac{2}{5}& \multicolumn{1}{l|}{\unitfrac{2}{5}}& g& \unitfrac{3}{5}& \multicolumn{1}{l|}{\unitfrac{3}{5}}& h& h& \multicolumn{1}{l|}{ \unitfrac{5}{5}}& \dots\\\hline
\dots &  $(\unitfrac{2}{5},\unitfrac{4}{5},\unitfrac{5}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & 0 &\unitfrac{2}{5}& \multicolumn{1}{l|}{\unitfrac{2}{5}}& g& g& \multicolumn{1}{l|}{\unitfrac{4}{5}}& h& h& \multicolumn{1}{l|}{ \unitfrac{5}{5}} & \dots\\\hline
\dots &  $(\unitfrac{3}{5},\unitfrac{4}{5},\unitfrac{5}{5})$  & \dots  & \multicolumn{1}{l|}{\dots} & 0 &0& \multicolumn{1}{l|}{\unitfrac{3}{5}}& g & g& \multicolumn{1}{l|}{\unitfrac{4}{5}}& h& h& \multicolumn{1}{l|}{ \unitfrac{5}{5}}& \dots\\\hline
\dots &  \dots  & \dots &\multicolumn{1}{l|}{\dots} & \dots & \dots & \multicolumn{1}{l|}{\dots} & \dots & \dots & \multicolumn{1}{l|}{\dots} & \dots & \dots & \multicolumn{1}{l|}{\dots}& \dots \\
\end{tabular}}
\end{table}

\begin{proof}
We first prove $r'(a',b'^{(i,j,k)})=a'^{(i,j)}\II[a'^{(i,j)}\leq \frac{k+j-1}{m}] + \frac{j-1}{m}\II[a'^{(i,j)}> \frac{k+j-1}{m}]$, then argue that it leads to $nsm$-approximability. 

For $j=1$, $b'^{(i,1,k)}=\frac{k}{m}e_i$. According to Definition \ref{defn:level}, when $a'^{(i,1)}>\frac{k}{m}$, all bidders are at the 0-th level, so
no bidder wins the item, and  $r(a',b'^{(i,j,k)})=0$. Otherwise, bidder $i$ wins the item, and pays $a'^{(i,1)}$. Thus, $r'(a',b'^{(i,1,k)})=a'^{(i,1)}\II[a'^{(i,1)}\leq \frac{k}{m}]$. For $j>1$, $b'^{(i,j,k)}=\frac{k+j-1}{m}e_i+\frac{j-1}{m}e_{n+1}$. Based on the third part of Definition \ref{ass:lebel}, bidder $n+1$ is at the $j$-th level. If $a'^{(i,j)}>\frac{k-j+1}{m}$, then bidder $n+1$ wins the item, and pays $r'(a',b'^{(i,j,k)})=\frac{j-1}{m}$. Otherwise, bidder $i$ wins the item, and pays $r'(a',b'^{(i,j,k)})=\frac{k+j-1}{m}$. Therefore, $r'(a',b'^{(i,j,k)})=a'^{(i,j)}\II[a'^{(i,j)}\leq \frac{k+j-1}{m}] + \frac{j-1}{m}\II[a'^{(i,j)}> \frac{k+j-1}{m}]$.




Next, we prove the approximability based on Lemma \ref{ass:single-out-2}. WLOG, consider one auction  $a'\in\A'$, and let $\Gamma^{\V,a'}$ be the row related to $a'$, which is a $ns(m-s+1)$-dimensional vector based on Lemma \ref{lem:level}. Our goal is to show that, there exists a vector $s$, such that 
$$ \forall \widehat{a}'\in \A', \widehat{a}'\not=a', \left\langle \Gamma^{\V,a'}-\Gamma^{\V,a},s\right\rangle\geq 1.$$
Denote $s^{(i,j,k)}$ as the  element of $s$ which is related to $b'^{(i,j,k)}$ (see Lemma \ref{lem:level}), and we discuss how to set $s^{(i,j,k)}$ as follows. 

First, based on the second part of Definition \ref{ass:lebel}, we have $\frac{j}{m}\leq a'^{(i,j)}\leq \frac{m-s+j}{m}$. Thus, combining  \eqref{eqn:v}, we know $\forall i\in[n]$,  $j\in[s]$, $\exists k'\in[m-s+1]$, such that $b'^{(i,j,k')}=a'^{(i,j)} e_i+\frac{j-1}{m}e_{n+1}$, which is in turn equivalent to $\frac{k'+j-1}{m}=a'^{(i,j)}$. In the column corresponding to this $b'^{(i,j,k')}$, $\forall \widehat{a}'\in\A'$, $\widehat{a}'^{(i,j)}\not=a'^{(i,j)}$, we have $r'({a}',b'^{(i,j,k')})-r'(\widehat{a}',b'^{(i,j,k')})\geq \frac{1}{m}.$ Intuitively, it means that, in this column, only the auctions whose $j$-th threshold for the $i$-th bidder equals to $a'^{(i,j)}$ yields the highest revenue, and the gap compared to other auctions is at least $\frac{1}{m}$. Thus, choosing the corresponding  $s^{(i,j,k')}$ as $m$, and setting $s^{(i,j,k)}=0$ for $k\not=k'$, makes $\sum_{k=1}^{m-s+1}r'({a}',b'^{(i,j,k)})s^{(i,j,k)}-r'(\hat{a}',b^{(i,j,k)})s^{(i,j,k)}\geq 1$. Since  we need  to ensure that the loss gap between $a'$ and any other auctions by at least 1, we need to repeat the aforementioned procedure for any $i\in[n]$, $j\in [s]$ and set $s^{(i,j,k')}=m$. Thus $\|s\|_1=nsm$ and $\Gamma^{\V}$ is $nsm$-approximable according to Lemma \ref{ass:single-out-2}.
% Note that Definition \ref{ass:lebel} ensures that every two auctions in $\A'$ differs by at least one element, so  repeat this operation for $i\in[n]$ and $j\in [s]$ makes the loss gap between $a'$ and any other auctions by at least 1, and this implies $nsm$-approximability according to Lemma \ref{ass:single-out-2}.

To help understanding, we provide an example for the case where $m=5$ and $s=3$ in Table \ref{tab:exp}. Here, each $a'^{(i,j)}$ is encoded by $m-s+1=3$ columns. We use $m-s+1=3$ columns to represent each $a'^{(i,j)}$. There exists one out of three columns (denoted by $k'$), where auctions with $a'^{(i,j)}=\frac{k'+j-1}{m}$ can get the largest revenue. And the corresponding revenue is at least $\frac{1}{m}$ better than auctions such that $\widehat{a}'^{(i,j)}\not=a'^{(i,j)}$.
% value, $\frac{k'+j-1}{m}=a'^{(i,j)}$

% For $a'^{(i,j)}=c$, there exists one out of three columns, where auctions with $a'^{(i,j)}=c$ has the largest value, and the gap w.r.t. others are at least $1/m$. 
\end{proof}
Combining Lemma \ref{lem:level}, Corollary \ref{cor:imp}, we get the following results. 
\begin{cor}
\label{cor:imp:3}
Consider running Algorithm \ref{alg:GFTPL:33} with $\Gamma^{\V}$ on the augmented problem. Let $\{a'_t\}_t\in\A'^T$ be the output of the algorithm, and  $\{a_t\}_t\in\A^T$ be the corresponding auctions in the original problem. Then Algorithm \ref{alg:GFTPL:33} is oracle-efficient, and
\begin{equation}
    \begin{split}
        \E\left[\sum_{t=1}^T r(a^*,b_t)-\sum_{t=1}^Tr(a_t,b_t)\right]= {} &O\left(\max\left\{nsm,ns\ln m, \sqrt{nms\cdot ns\ln m}\right\}\sqrt{T-L_T^*}\right) \\
        = {} & O\left(nsm\sqrt{T-L_T^*}\right).
    \end{split}
\end{equation}
$$$$
\end{cor}

%Specifically, let $\A=\{\frac{1}{m},\dots,\frac{m}{m}\}^{ns}$ be the set of possible auctions. In each round $t$, an auctioneer picks a auction $a\in\A$, where we let $a=[a^{(1,1)},\dots,a^{}]$


%To understand the auction setting, imagine a seller wants to sell $r$ items to $n$ bidders.  Each bidder has a combinatorial utility function $v_i:\{0,1\}^r\rightarrow [0,1]$ and
% gets an allocation $q_i\in\{0,1\}^r$. We assume the bidding process is truthful, which means that each bidder can maximize his utility by reporting his true valuation $v_i$. We use $v$ to denote the valuation profile as well as the bidding profile. Therefore, the utility of the bidder would be $v_i(q_i(v))-p_i(v)$.
 
 
%In each round $t$ of the this setting, firstly an auctioneer chooses an auction $a_t$ from a discretized auction set $\A$ of cardinality $K$. After that, she receives a bidder profile $v_t\in\V$, and gains a reward $r(a_t,v_t)$, where $r:\A\times\V\mapsto[0,1]$. 
%An auction $a$ receives the valuation profiles from all bidders and determines how to allocate the items and how much to charge each bidder. We use $r(a,v)$ to denote the revenue of auction $a$ w.r.t. valuation profile $v$. In the online auction setting, we assume each $a\in\mathcal{A}$ and $v\in\mathcal{V}^n$ where $\mathcal{A}$ denotes all truthful auctions and $\mathcal{V}$ denotes all possible valuations. For each $t=1,\dots, T$, the learner chooses an auction $a_t$ while the adversary chooses a valuation profile $v_t$, then the learner gets to know $v_t$ and receives the revenue $r(a_t,v_t)$. The goal of the learner is to compete the revenue earned by the best auction in hindsight.


%To deal with auction problems, we first translate Algorithm \ref{alg:GFTPL:main} to the online learning with rewards setting, i.e., in each round $t$, after choosing $a_t$, instead of suffering a loss, the learner obtains a reward $r(a_t,v_t)$, where $r:\A\times\V\mapsto[0,1]$, and the 
%{regret} is defined as









%\begin{lemma}
%Assume there exists $s^{(k)}$ such that
%$$
%\langle\Gamma^{(k)}-\Gamma^{(j)},s^{(k)}\rangle=f(x^{(k)},y)-f(x^{(j)},y)
%$$
%holds for any $y\in|\mathcal{Y}|$, $k\in[K]$ and %$j\neq k$, then we can get the small-loss bound %$O({N}^{\frac{1}{4}}{(\ln %K)}^{\frac{1}{4}}L_T^{*\frac{1}{2}})$.
%\end{lemma}


% For this problem, we can also use all contexual vectors to construct $\Gamma$ and get $O(\sqrt{|P|\ln|\Sigma|L_T^{\star}})$ regret.
% the $\Gamma$ matrix of \cite{dudik2020oracle} satisfies 
% $O({|\mathcal{P}|}^{\frac{1}{4}}{\ln |\Sigma|}^{\frac{1}{4}}L_T^{*\frac{1}{2}})$
\subsection{Other applications}
% Apart from online auctions, our methods also apply to the following settings. 
\label{subsection:other:application}
\paragraph{Oracle learning and finite parameter space} In 
many real-world applications, such as security game \citep{balcan2015commitment} and online bidding with finite threshold vectors \citep{daskalakis2016learning}, the decision set $\X$ is extremely large, while the adversary's action set $|\Y|$ is finite small. For these problems, we can construct an implementable PTM based the following Lemma, where the proof can be found in Appendix \ref{app:proof:lem:smally}. 
\begin{lemma}
\label{lem:small:y}
Consider the setting with $|\Y|=d$ ($d\ll K$), then there exists a $1$-approximable and implementable $\Gamma$ with $d$ columns and complexity 1. 
\end{lemma}
Combining Lemma \ref{lem:small:y} and Theorem \ref{thm:main:11}, and configuring $c=\sqrt{\max\{\ln K,\sqrt{d\ln K}\}}$, 
we observe that our algorithm achieves  $O(\sqrt{\max\{\ln K,\sqrt{d\ln K}}\}\sqrt{L_T^*})$ small-loss bound. On the other hand, in this kind of problems, because of the continuity of the loss functions, a $\delta$-admissible PTM in general does not exist (as $\delta$ may approach 0 without any discretization). Therefore, our proposed condition not only leads to a tighter bound, but can also solve problems that the original GFTPL \citep{dudik2020oracle} can not handle. 


\paragraph{Transductive online classification} Finally, we consider the transductive online classification problem \citep{syrgkanis2016efficient,dudik2020oracle}. In this setting, $\X$ contains  $K$ binary classifiers. In each round $t$, firstly the adversary picks a feature vector $w_t\in \W$, where $|\W|=m$. Then, the learner chooses a classifier $x_t(\cdot)$ from $\X$. After that, the adversary reveals the label $y_t\in\{0,1\}$, and the learner suffers a loss $f(x_t,(w_t,y_t))=\mathbb{I}[x_t(w_t)\not=y_t]$. We assume the problem is transductive, i.e., the learner has access to $\W$ at the beginning. For this setting, we achieve the following results (the proof is in Appendix \ref{app:lem:5}).
\begin{lemma}
\label{lem:small}
Consider transductive online classification with $|\W|=m$. Then there exists a 1-approximable and implementable PTM with $m$ columns and complexity 1. Moreover, Algorithm \ref{alg:GFTPL:main} with such a PTM and appropriately chosen parameters achieves  $O(\sqrt{\max\{\ln K,\sqrt{m\ln K}}\}\sqrt{L_T^*})$ regret.
\end{lemma}
\paragraph{Negative implementability} In the this paper we assume that the offline oracle can solve the minimization problem in \eqref{eqn:oracle} given any real-weights. In some cases, the oracle can only accept positive weights. This problem can be solved by constructing negative implementable PTM \citep{dudik2020oracle}. Note that in most  cases discussed above negative implementable and approximable PTM exist, which is shown in Appendix \ref{app:negei}.

\section{Best-of-Both-Worlds Bound}
By setting all step sizes $\eta_t$ as $\infty$, Algorithm \ref{alg:GFTPL:main} reduces to the classical FTL algorithm, which  suffers  linear regret in the adversarial setting and enjoys much tighter bounds when the data is IID or number of leader changes is small.
To be more specific, we introduce the following regret bound for FTL.
\begin{lemma}[Lemma 9, \cite{de2014follow}]
\label{lem:ftl}
Let $x_t^{\emph{\FTL}}=\argmin_{i\in[K]} \sum_{s=1}^{t-1}f(x^{(i)},y_s)$ be the output of the FTL algorithm at round $t$, $C_T$ the set of rounds where the leader changes, and $\delta_t=f(x^{\emph{\FTL}}_t,y_t)-(L_t^{*}-L_{t-1}^*)$ the ``mixability gap'' at round $t$. Then for any $T\geq1$, the regret of FTL is bounded by 
$ R_T^{\emph{\FTL}}\leq \sum_{t\in C_T}\delta_t\leq |C_T|.$
\end{lemma}
Note that since $f\in[0,1]$ and $L_t^*-L_{t-1}^*\in[0,f(x^{\emph{\FTL}}_t,y_t)]$, we know $\delta_t\in[0,1]$. For the \textit{i.i.d} case, if the mean loss of the best expert is smaller than that of other experts by a constant, then due to the law of large numbers, the number of leader changes would be small, which results in a constant regret bound \citep{de2014follow}. 

Denote $U_T^{\FPL}$ as the attainable regret bound (as in Theorem \ref{thm:main:11}) for running  Algorithm \ref{alg:GFTPL:main} alone and $U_T^{\emph{\FTL}}=\sum_{t\in C_T}\delta_t$ to be that of FTL. In the following, we develop a new algorithm and prove that it is optimal in both worlds, that is, its regret is on the order of  $O(\min\{U_T^{\FTL},U_T^{\FPL}\})$.

\begin{algorithm}[t]
\caption{Oracle-efficient Flipflop (OFF)}
\textbf{Initialization:} $\textsf{Alg}_1=\textsf{FTL}$
\begin{algorithmic}[1]
\label{alg:GFTPL}
\FOR{$t=1,\dots,T$}
\STATE Get $x_t$ by $\textsf{Alg}_t$, observe $y_t$
\STATE Compute $\widehat{U}_t^{\FTL}$ and $\widehat{U}_t^{\FPL}$
\IF{$\textsf{Alg}_t==$ FTL and $\widehat{U}_t^{\FTL}>\alpha \widehat{U}_t^{\FPL}$}
\STATE $\Alg_{t+1} =$ GFTPL
\ELSIF{$\textsf{Alg}_t==$ GFTPL and $\widehat{U}_t^{\FPL}>\beta \widehat{U}_t^{\FTL}$}
\STATE $\Alg_{t+1} =$FTL
\ENDIF 
\STATE Feed $y_t$ to $\Alg_{t+1}$
\ENDFOR
\end{algorithmic}
\end{algorithm}
The proposed algorithm, named as oracle-efficient flipflop (OFF) algorithm, is summarized in Algorithm \ref{alg:GFTPL}. It is motivated by the Flipflop algorithm \citep{de2014follow}, and the core idea is to switch between FTL and GFTPL (Algorthm \ref{alg:GFTPL:main}) based on the comparison of the estimated regret. We optimistically start from FTL. In each round $t$, we firstly pick $x_t$ based on the current algorithm $\Alg_t$, and then obtain the adversary's action $y_t$ (line 2). Next, we compute the estimated bounds of regret of both algorithms until round $t$ (line 3). Specifically, let $\I_t^{\FTL}=\{i|i\in[t], \Alg_i=\text{FTL}\}$ and $\I_t^{\FPL}=\{i|i\in[t], \Alg_i=\text{GFTPL}\}$
be the set of rounds up to $t$ in which we run FTL and GFTPL. Then, the estimated regret of FTL in $\I_t^{\FTL}$ is given by 
$\widehat{U}_t^{\FTL}=\sum_{i\in\I_t^{\FTL}}\delta_i,$
and 
the estimated regret of GFTPL in $\I_t^{\FPL}$ can be bounded via Theorem \ref{thm:main:11}: 
\begin{equation}
    \begin{split}
\widehat{U}^{\FPL}_t= {} & \left({4\sqrt{2}\max\{2\ln K,\sqrt{N\ln K}\}}
+{4\gamma}\right) \sqrt{\widehat{L}_t^*+1}\\
{} & + {8\gamma}\ln\left(\sqrt{\widehat{L}_t^*+1}+\gamma\right) + 2\gamma^2 + 4\sqrt{2}\max\{2\ln K,\sqrt{N\ln K}\}\gamma.
  \end{split}
\end{equation}
where $\widehat{L}_t^*=\min_{x\in \X}\sum_{i\in{\I}_t^{\FPL}}f(x,y_i)$ and we set $c=1$. Note that, the two quantities defined above are the exact regret upper bounds of the two algorithms on their sub-time intervals up to round $t$, due to the fact that the regret bounds provided in Lemma \ref{lem:ftl} and Theorem \ref{thm:main:11} are \emph{timeless}. Moreover, note that the two values can be computed by the oracle. We compare the estimated regret of both algorithms, and use the algorithm which performs better for the next round (lines 4-8).  %Essentially, it can be considered as running FTL and GFTPL in parallel: In each round, we only feed the better algorithm with the loss function, and choose its output. 

For the proposed algorithm, we have the following theoretical guarantee (the proof can be found in Appendix \ref{E}). 
\begin{theorem}
\label{thm:off}
Assume we have a $\gamma$-approximable $\Gamma$, then Algorithm \ref{alg:GFTPL} is able to achieve the following bound: 
$$ R_T^{\OFF}\leq \min\left\{3 U_T^{\FPL}+1, 3{U}_T^{\FTL}+\tau\right\},$$
where $\tau={4\sqrt{2}\max\{2\ln K,\sqrt{N\ln K}\}}
+{12\gamma}$ and $\alpha=\beta=1$.
\end{theorem}

%\section{Best-of-Both-Worlds-v2}
%\begin{algorithm}[t]
%\caption{Hedge with non-uniform weights}
%\textbf{Initialization:} Expert set %$S=\{{E_1=\FTL,E_2=\FPL}\}$, Initial weights: %$w_{1,1}=\frac{1}{\exp(\frac{1}{T})}$, %$w_{2,1}=1-w_{1,1}$.
%\begin{algorithmic}[1]
%\label{alg:GFTPL}
%\FOR{$t=1,\dots,T$}
%\STATE Receive $x_{t,i}$ from each expert $E_i\in S$
%\STATE Choose $x_t$ by: $\P[x_t=x_{t,i}]=w_{t,i}$. 
%\STATE 
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}
%Next, we consider obtain similar results as in Theorem \ref{thm:off} by using a meta-algorithm (such as Hedge) to combining \FPL\ and \FTL. Our ideal meta-algorithm should achieve:
%$$L_T-L_{T}^i\leq O\left(\sqrt{L_T^i\ln\frac{1}{w_{1,i}}}\right)$$
%regret for each expert $i$, where $w_{1,i}$ is the initial weight.

==> intro.tex <==
\section{Introduction}

Online learning is a fundamental paradigm for modeling sequential decision making problems \citep{bianchi-2006-prediction,Online:suvery,Intro:Online:Convex}. 
Online learning is usually formulated as a zero-sum game between a learner and an adversary.
In each round $t=1,\dots,T$, the learner first picks an action $x_t$ from a (finite) set $\X=\{x^{(1)},\dots,x^{(K)}\}$ with cardinality equal to $K$. In the meantime, an adversary reveals its action $y_t\in\Y$. As a consequence, the learner observes $y_t$, and suffers a loss $f(x_t,y_t)$, where $f:\X\times\Y\mapsto[0,1]$. The goal is to minimize the \emph{regret}, which is defined as the difference between the cumulative loss of the learner $\sum_{t=1}^T f(x_t,y_t)$, and the cumulative loss  of the best action in hindsight $L_T^*=\min_{x\in\X}\sum_{t=1}^T f(x,y_t)$.

A wide variety of algorithms have been proposed for the goal of minimizing worst-case regret (without any consideration of computational complexity per iteration); see~\citep{bianchi-2006-prediction,Online:suvery,Intro:Online:Convex} for representative surveys of this literature.
These algorithms all obtain a worst-case regret bound of the order $O(\sqrt{T \log K})$, which is known to be minimax-optimal~\citep{bianchi-2006-prediction}.
% However, classical online algorithms suffer from twin shortcomings: a) they do not adapt, on-the-fly, to friendlier data structure when it exists, and b) they are inefficient at scale as their computational complexity per iteration is linear in $K$.
% While a) and b) have been addressed independently (as detailed below), there does not exist an online learning algorithm that is in general data-adaptive \emph{and} scalable.
% The central goal of this paper is to design such an algorithm.
% In the literature, a great deal of algorithms have been proposed for online learning  \citep{bianchi-2006-prediction}. Many of them can obtain a regret bound of order $O(\sqrt{T\log K})$, which has been shown to be \emph{worst-case optimal}, in a strong sense that for certain instances an $\Omega(\sqrt{T\log K})$ lower bound is unavoidable. 
Over the last two decades, sophisticated adaptive algorithms have been designed that additionally enjoy \emph{problem-dependent} performance guarantees,
which can automatically lead to better results in friendly environments. One of the most important example for this kind of guarantees is the so-called ``small-loss'' bound \citep{hutter2005adaptive,bianchi-2006-prediction,van2014follow}. Such a bound  depends on the best cumulative loss in hindsight (i.e. $L_T^*$) instead of the total number of rounds ($T$).
Thus, this bound is much  tighter than the worst-case bound, especially when the best decision performs well in the sense of incurring a very small loss. Another example is the ``best-of-both-worlds'' bound \citep{van2014follow}, which results in an even tighter regret bound for independent and identically distributed (IID) loss functions. 

However, all of these algorithms applied out-of-the-box suffer a \emph{linear} dependence on the number of decisions $K$.  This is prohibitively expensive, especially in problems such as network routing \citep{awerbuch2008online} and combinatorial market design \citep{cesa2014regret}, where the cardinality of the decision set grows exponentially with the natural expression of the problem. Although several efficient algorithms do exist when the loss functions have certain special structure, such as linearity~\citep{kalai2005efficient}, or convexity~\citep{zinkevich-2003-online}, these results can not be easily extended to the more general settings of interest.

Notice that the efficiency of the above specialized methods is usually made possible by assuming that the corresponding \emph{offline} optimization problem (i.e., minimizing the (averaged) loss) can be solved efficiently. This observation motivates the \emph{oracle-efficient online learning} problem \citep{hazan2016computational}.
In this setting, the learner has access to a black-box offline oracle, which, given a real-weighted dataset $\S=\{(w^{(j)},y^{(j)})\}_{j=1}^n$,
can efficiently return the solution to the following problem: 
\begin{equation}
\label{eqn:oracle}
  \argmin\limits_{x\in\X} \sum_{j=1}^n w^{(j)}f(x,y^{(j)}).
\end{equation}
The goal  is to design \emph{oracle-efficient} algorithms which can query the offline-oracle $O(1)$ times each round.  Concrete examples of such an oracle include algorithms for empirical
risk minimization \citep{PRML}, data-driven market design \citep{nisan2007computationally}, and dynamic programming \citep{bertsekas2019reinforcement}.  

As pointed out by \cite{hazan2016computational}, the design of oracle-efficient algorithms is extremely challenging and such an algorithm does not exist in the worst case. Nevertheless, recent work \citep{daskalakis2016learning,syrgkanis2016efficient,dudik2020oracle} has introduced a series of algorithms which are oracle-efficient when certain  sufficient conditions are met. 
Among them, the state-of-the-art method is the \emph{generalized-follow-the-perturbed-leader} algorithm~\citep[GFTPL,][]{dudik2020oracle}, which is a variant of the  classical follow-the-perturbed-leader (FTPL) algorithm \citep{kalai2005efficient}. Similar to FTPL, GFTPL perturbs the cumulative loss of each decision by adding a random variable, and chooses the decision with the smallest perturbed loss as $x_t$. However, the vanilla FTPL perturbs each decision independently, which requires to generate $K$ independent random variables in total. Moreover, the oracle in \eqref{eqn:oracle} can not be applied here since the oracle can not handle the perturbation term. To address these limitations, GFTPL only generates a low-dimensional noise vector in the beginning, and constructs $K$ \emph{dependent} perturbations based on the multiplication between the noise vector and  a \emph{perturbation translation matrix} (PTM). In this way, the computational complexity for the noise generation is largely reduced. On the other hand, oracle-efficiency can be achieved by setting the elements in the PTM as carefully designed synthetic losses.
\cite{dudik2020oracle} show that a worst-case optimal regret bound can be obtained when the PTM is \emph{admissible}, i.e., every two rows are significantly distinct. This serves as a \emph{sufficient condition} for achieving oracle-efficiency. 

While these results form a solid foundation for general \emph{worst-case} oracle-efficient online learning, it remains unclear whether \emph{problem-dependent}, or \emph{data-adaptive} bounds are achievable in conjunction with oracle-efficiency.
%  when PTM is \emph{admissible}, i.e., 
% has significantly different rows. Moreover, if PTM can be constructed by a small set of loss vectors, GFTPL yields oracle-efficiency. This serves as the \emph{sufficient condition} for achieving oracle-efficiency.
%Unlike FTPL, GFTPL generates a low-dimensional noise vector in the beginning, and linearly combines its components via a \emph{perturbation translation matrix} (PTM), which is delicately constructed by a small set of loss vectors. GFTPL also picks the decision based on the perturbed learning history but the perturbations are \emph{dependent}. Since the PTM is constructed by losses, the offline oracle can be invoked to get the best decision, while the computational complexity for the noise generation is largely reduced. Hence GFTPL is oracle-efficient. Further, if the PTM is  \emph{admissible}, i.e., 
%has significantly different rows, then GFTPL attains a \emph{worst-case optimal} regret bound. The admissibility serves as the \emph{sufficient condition} for achieving oracle-efficiency.
%The vanilla FTPL perturbs the cumulative loss of each decision independently via a  random variable,
%Similar to FTPL, GFTPL perturbs the cumulative loss of each decision by a random variable, and chose the decision with the best perturbed cumulative loss. However, the vanilla FTPL is inefficient (except for linear losses), since it perturbs the cumulative loss of each decision independantly, 
%typically requires 
%The vanilla FTPL algorithm generates an \emph{independent} perturbation for each decision, and choose the best decision according to its perturbed cumulative loss. This is inefficient in general, because it not only need to generate $K$ random variables for perturbation, but also break 
%thus is computationally inefficient . Unlike FTPL, GFTPL generates a low-dimensional noise vector in the beginning and linearly combines its components via a \emph{perturbation translation matrix} (PTM), which is delicately constructed by a small set of loss vectors. GFTPL also picks the decision based on the perturbed learning history but the perturbations are \emph{dependent}. Since the PTM is constructed by losses, the offline oracle can be invoked to get the best decision, while the computational complexity for the noise generation is largely reduced. Hence GFTPL is oracle-efficient. Further, if the PTM is  \emph{admissible}, i.e., 
%has significantly different rows, then GFTPL attains a \emph{worst-case optimal} regret bound. The admissibility serves as the \emph{sufficient condition} for achieving oracle-efficiency.
% Similar to FTPL, GFTPL picks the decision based on the perturbed learning history. However, the vanilla FTPL is  inefficient in general (except for linear functions), since it usually requires to generate $K$ noises for perturbation. Moreover, the form of perturbation also makes the oracle unappliable. To address these limitations, GFTPL only generates a low-dimensional noise vector in the beginning, and then spreads the linear combination of the noises across all decisions through a \emph{perturbation translation matrix} (PTM). In this way, the computational complexity for the noise generation is largely reduced. A \emph{worst-case optimal} regret bound is obtained 
%  when PTM is \emph{admissible}, i.e., 
% has significantly different rows. Moreover, if PTM can be constructed by a small set of loss vectors, GFTPL yields oracle-efficiency. This serves as the \emph{sufficient condition} for achieving oracle-efficiency.
In other words, the design of a generally applicable oracle-efficient \emph{and} adaptive online learning algorithm has remained open. 
% Although the algorithmic and theoretical foundations for general oracle-efficient online learning are beginning to take shape, it's still unclear whether \emph{problem-dependent} bound is achievable. 
In this paper, we provide an affirmative answer to this problem, and make the following contributions. 
%for  in oracle-efficient online learning begining to take 
%Following this line of research, we ask whether improved regret bounds can be obtained in an oracle-efficient fashion. In particular, we are interested in the \emph{small-loss bound}, i.e., the bound of form
%$O(\sqrt{L_*})$ . Such a guarantee reduces to $O(\sqrt{T})$ in the worst case, while becoming much tighter when the best expert performs well. Moreover, the small-loss bound can be obtained inefficiently \citep{hutter2005adaptive,de2014follow}, but whether it can be achieved in the general oracle-efficient setting remains open. In this paper, we provide an affirmative answer to this question, and make the following contributions:
\begin{itemize}
    \item We propose a variant of the GFTPL algorithm~\citep{dudik2020oracle}, and derive a new sufficient condition for 
    ensuring oracle-efficiency while achieving the \emph{small-loss} bound. 
    % We note that the admissibility condition of the PTM that is used in GFTPL is not sufficiently strong to produce a small-loss bound (and include explicit counterexamples for the same).
    Our key observation is that while the admissibility condition of the PTM in GFTPL successfully stabilizes the algorithm (by ensuring that $\P[x_t\not=x_{t+1}]$ is small), it is too weak to adapt to a small loss.
    We address this challenge via a new condition for PTM, called approximability. Critically, this condition ensures 
    %Intuitively, it ensures the linear combination of the columns of the matrix is a good approximation of the loss vector, in the sense that the oracle behaves similarly when taking the two as input. Under the proposed condition,
    a stronger stability measure, i.e., the ratio of $\P[x_t=x^{(i)}]$ and $\P[x_{t+1}=x^{(i)}]$ is upper-bounded by a universal constant for any $i\in[K]$. We obtain the small-loss bound by equipping GFTPL with an approximable PTM, a data-dependent step-size and Laplace distribution for the perturbation noise. 
    Our new condition of \emph{approximability} is simple and interpretable, and can be easily verified for an arbitrary PTM. 
    It shares both similarities and differences from the \emph{admissibility} condition proposed in~\cite{dudik2020oracle}.
    % We note that, our new condition is related but distinct from admissibility. 
    We demonstrate this through several examples where one of the sufficient condition holds, but not the other.  
    
    \item We identified a series of real-world applications where  approximable PTMs exist, for example: (a) a series of online auctions problems \citep{dudik2020oracle}; (b) problems with a small adversary's action space $|\Y|$ \citep{daskalakis2016learning};  and (c) transductive online classification \citep{syrgkanis2016efficient,dudik2020oracle}. This is the first-time that the small-loss bound is obtained in these applications.
    To achieve this, we introduce novel PTMs and analysis for showing the approximability condition on these PTMs.
    % and proving the conditions in several cases is highly non-trivial. 
    \item We achieve the ``best-of-both-worlds'' bound, which enjoys even tighter results when the data is IID or the number of leader changes is small. The main idea is to  combine our proposed algorithm with vanilla FTL leveraging ideas from a meta-algorithm introduced in~\cite{van2014follow}.   
\end{itemize}

==> related_work.tex <==
\section{Related Work}
Our work contributes to two classes of problems: oracle-efficient online learning and adaptive online learning. In this section, we briefly review the related work in these areas. 

\subsection{Oracle-efficient online learning}
For oracle-efficient online learning, the pioneer work of \cite{hazan2016computational} points out that oracle-efficient methods do not exist when dealing with general hostile adversaries, which implies that additional assumptions on the problem structure have to be made. \cite{daskalakis2016learning} consider the setting in which the cardinality of the adversary's action set $\Y$ is finite and small, and propose to add a series of ``fake'' losses to the learning history based on random samples from $\Y$. They prove that for this setting an $O(|\Y|\sqrt{T})$ bound can be obtained.  \cite{syrgkanis2016efficient} study the contextual combinatorial online learning problem, where each action is associated with a binary vector. They also assume the loss function set contains all linear functions as a sub-class. For this problem, \cite{syrgkanis2016efficient} construct a set of synthetic losses for perturbation based on randomly-selected contexts, and achieve worst-case optimal bounds when all the contextual information can be obtained beforehand, or when there exists a small set of contexts that can tell each decision apart. \cite{dudik2020oracle} focus on the general non-contextual setting, and propose the generalized FTPL algorithm.
This algorithm generates a small number of random variables at the beginning, and then 
perturbs the learning history via the linear combinations of these random variables. The algorithm can be implemented efficiently by setting the combination parameters as carefully designed loss values. \cite{niazadeh2021online} consider a more complicated combinatorial setting where the offline problem is NP-hard, but a robust \emph{approximation} oracle exists. For this case, they propose an online algorithm based on the approximation oracle, and prove that it has low approximate regret, which is a measure weaker than regret. 
Note that the aforementioned methods suffer from the worst-case bounds, and cannot benefit from nice structures in data. Recently, several concurrent work \citep{block2022smoothed,haghtalab2022oracle} investigate how to obtain tighter bounds oracle-efficiently when the distribution of data is close to the uniform distribution \citep{rakhlin2011online,haghtalab2022smoothed}. However, their results do not improve the dependence on $T$. 

In this paper, we mainly focus on the so-called  the learning with expert advice setting \citep{bianchi-2006-prediction}, where the action set is discrete, and the loss can be highly non-convex. On the other hand, efficient algorithms can be obtained when the loss functions have certain properties, such as linearity  \citep{kalai2005efficient,hutter2005adaptive,awerbuch2008online}, convexity \citep{zinkevich-2003-online,Hazan:2007:log} or submodularity \citep{Online:Submodular}.  Finally, we note that,  in this paper we mainly focus on the full-information setting, where the learner can observe the whole loss function after the action is submitted. On the other hand, online learning with oracle has also been  widely studied in the bandit setting \citep{NIPS2007_3178,10.5555/3020548.3020569,agarwal2014taming,foster2018practical,foster2020beyond}. 

\subsection{Adaptive online learning}
In this paper, we focus on designing oracle-efficient algorithms with \emph{problem-dependent} regret guarantees. Note that this kind of bound can be achieved by many inefficient algorithms in general, such as Hedge and its variants \citep{bianchi-2006-prediction,de2014follow,pmlr-v40-Luo15}, and follow-the-perturbed-leader \citep{van2014follow} or follow-the-regularized-leader \citep{orabona2019modern} type of methods. Small-loss can also be obtained efficiently when the loss functions are simply linear \citep{hutter2005adaptive,syrgkanis2016efficient}. On the other hand, in online convex optimization, i.e., when the decision set and the loss functions are convex, 
small-loss bound can be obtained when the loss functions  are smooth \citep{NIPS2010_Smooth,Beyond:Logarithmic,AAAI:2020:Wang}.
However, these algorithms heavily rely on the special structure of the loss functions.
In this paper, we take the first step to extend these methods to support the complicated and non-convex problems which appear in real-world applications.  

Apart from the small-loss, there exist other types of problem-dependent bounds, such as second-order bound \citep{Cesa-Bianchi2005,gaillard2014second}, or quantile bound \citep{chaudhuri2009parameter,pmlr-v40-Koolen15a}, but how to obtain these more refined theoretical guarantees in the oracle-efficient setting remains an open problem. 
